Perfectly Balanced: Improving Transfer and Robustness of Supervised Contrastive Learning

An ideal learned representation should display transferability and robustness. Supervised contrastive learning (SupCon) is a promising method for training accurate models, but produces representations that do not capture these properties due to class collapse -- when all points in a class map to the same representation. Recent work suggests that "spreading out" these representations improves them, but the precise mechanism is poorly understood. We argue that creating spread alone is insufficient for better representations, since spread is invariant to permutations within classes. Instead, both the correct degree of spread and a mechanism for breaking this invariance are necessary. We first prove that adding a weighted class-conditional InfoNCE loss to SupCon controls the degree of spread. Next, we study three mechanisms to break permutation invariance: using a constrained encoder, adding a class-conditional autoencoder, and using data augmentation. We show that the latter two encourage clustering of latent subclasses under more realistic conditions than the former. Using these insights, we show that adding a properly-weighted class-conditional InfoNCE loss and a class-conditional autoencoder to SupCon achieves 11.1 points of lift on coarse-to-fine transfer across 5 standard datasets and 4.7 points on worst-group robustness on 3 datasets, setting state-of-the-art on CelebA by 11.5 points.

==> figs/L_spread_tsne.tex <==
\begin{figure*}[t]
  \includegraphics[width=7.25in]{figs/L_spread_embs_vs_L_SC.pdf}
  \centering
  \caption{
    $L_{spread}$ produces embeddings that are qualitatively better
    than those produced by $L_{SC}$.
    We show t-SNE visualizations of embeddings for the CIFAR10 test set and
    report cosine similarity metrics (average intracluster cosine similarities,
    and similarities between individual points and the class cluster).
    $L_{spread}$ produces lower intraclass cosine
    similarity and embeds images from rare strata
    further out over the hypersphere
    than $L_{SC}$.
  }
  \label{fig:L_spread_tsne}
\end{figure*}


==> figs/homotopy_cifar100.tex <==
\begin{figure}[t]
  \centering
  % Synthetic Validation of Geometric Properties of Strata on CIFAR100 \\
  \includegraphics[width=2.5in]{figs/geometric_synthetic.pdf}
  % \includegraphics[height=1.25in]{figs/homotopy_cifar100.png}
  % \includegraphics[height=1.25in]{figs/homotopy_cifar100_tsne.png}
  \caption{
    Points from large subclasses cluster tightly; points
    from small subclasses scatter (CIFAR100-Coarse, unbalanced subclasses).
  }
  \label{fig:homotopy_cifar100}
\end{figure}


==> sections/method.tex <==
%!TEX root = ../main.tex

\section{\sysname}
\label{sec:method}

We use our theoretical insights to propose a new method \sysname. This method uses $\lspread$ (consisting of augmentations) concatenated with a class-conditional autoencoder.

==> tables/quality.tex <==
%!TEX root = ../main.tex

\begin{table}[t]
     \centering
     \begin{tabular}{lccclccc}
         \toprule                   & \multicolumn{3}{c}{\textbf{End Model Perf.}}  \\ \cmidrule(lr){2-4}
         \textbf{Dataset}           & $L_{SS}$       & $L_{SC}$       & $L_{spread}$  \\ \midrule
         \textbf{CIFAR10}           & 89.7           & 90.9           & \textbf{91.5} \\
         \textbf{CIFAR10-Coarse}    & 97.7           & 96.5           & \textbf{98.1} \\
         \textbf{CIFAR100}          & 68.0           & 67.5           & \textbf{69.1} \\
         \textbf{CIFAR100-Coarse}   & 76.9           & 77.2           & \textbf{78.3} \\
         \textbf{CIFAR100-Coarse-U} & 72.1           & 71.6           & \textbf{72.4} \\
         \textbf{MNIST}             & 99.1           & \textbf{99.3}  & 99.2          \\
         \textbf{MNIST-Coarse}      & 99.1           & \textbf{99.4}  & \textbf{99.4} \\
         \textbf{Waterbirds}        & 77.8           & 73.9           & \textbf{77.9}  \\
         \textbf{ISIC}              & 87.8           & 88.7           & \textbf{90.0} \\
         \bottomrule
     \end{tabular}

\caption{
    End model performance training with $L_{spread}$ on various datasets compared
    against contrastive baselines.
    All metrics are accuracy except for ISIC (AUROC).
    $L_{spread}$ produces the best performance in \num{7} out of \num{9}
    cases, and matches the best performance in \num{1} case.
}
\label{table:quality}
\end{table}

